Estimating Discrete Total Curvature with Per Triangle Normal Variation

We introduce a novel approach for measuring the total curvature at every triangle of a discrete surface. This method takes advantage of the relationship between per triangle total curvature and the Dirichlet energy of the Gauss map. This new tool can be used on both triangle meshes and point clouds and has numerous applications. In this study, we demonstrate the effectiveness of our technique by using it for feature-aware mesh decimation, and show that it outperforms existing curvature-estimation methods from popular libraries such as Meshlab, Trimesh2, and Libigl. When estimating curvature on point clouds, our method outperforms popular libraries PCL and CGAL.

==> conclusion.tex <==
We present a novel, \mob{}-equivariant spherical convolution operator which we call \textit{\mob{} convolution}. With it, we develop the foundations for \mob{}-equivariant spherical CNNs and demonstrate the utility of this framework by achieving strong results in both geometry and spherical-image processing tasks.   

More generally, this work represents an effort to move both image and surface convolutional neural networks beyond standard rotation- and isometry-equivariance and into the realm of conformal-equivariance. In particular, our experiments suggest that the latter transition may be especially relevant in the context of shape analysis and recognition and we hope this work serves to catalyze the development of a new generation of surface networks better able to handle the kinds of complex deformations found in real-world shape data. 
